A Hybrid Approach to Formal Verification of Higher-Order Masked Arithmetic Programs

Side-channel attacks, which are capable of breaking secrecy via side-channel information, pose a growing threat to the implementation of cryptographic algorithms. Masking is an effective countermeasure against side-channel attacks by removing the statistical dependence between secrecy and power consumption via randomization. However, designing efficient and effective masked implementations turns out to be an error-prone task. Current techniques for verifying whether masked programs are secure are limited in their applicability and accuracy, especially when they are applied. To bridge this gap, in this article, we first propose a sound type system, equipped with an efficient type inference algorithm, for verifying masked arithmetic programs against higher-order attacks. We then give novel model-counting based and pattern-matching based methods which are able to precisely determine whether the potential leaky observable sets detected by the type system are genuine or simply spurious. We evaluate our approach on various implementations of arithmetic cryptographicprograms.The experiments confirm that our approach out performs the state-of-the-art base lines in terms of applicability, accuracy and efficiency.

==> finite-set-constraint.tex <==

\subsection{Q2: Handling Combinatorial Explosion of Observable Sets} \label{sec:divconq}
Exhaustive enumeration of all the subsets of observable variables with size up to $d$  may not scale %quickly become intractable
when $d$ and $X_o$ grow, whereas we present a divide-and-conquer algorithm %for verifying order-$d$ probing secure,
inspired by the prior work %of Barthe at al.~
\cite{BBDFGS15}. Recall the following two simple observations.
\begin{description}
	\item[Observation 1:] If $\vdash \Oo:\sid$ is valid, then $\vdash \Oo':\sid$ is valid for all $\Oo'\subseteq \Oo$ (cf. Proposition~\ref{prop:uniform2SI}(2)).
	\item[Observation 2:] If $\bigcup_{x\in\Oo_1}\Var({\Expr(x)})\subseteq X_p$ and $\vdash \Oo_2:\sid$ is valid,
then, $\vdash \Oo_1\cup\Oo_2:\sid$ is valid (cf. rule ({\sc Sid}$_1$) in Figure~\ref{tab:semrules}).
\end{description}


Based on Observation 1, our goal is to find %fewer, larger
sets $\Oo_1,\cdots,\Oo_m$ of observable variables such that $\vdash \Oo_j:\sid$ for all $ 1\leq j\leq m$,
and %they together can cover
for each size-$d$ set $\Oo\subseteq X_o$, $\Oo\subseteq \Oo_j$
for some $1\leq j\leq m$. As pointed out %by Barthe at al.
in \cite{BBDFGS15},
the latter condition is the contrapositive of the Hitting
Set problem, which is NP-hard. So we only aim to propose practically efficient algorithms.

Based on Observation 2, we can isolate the set of variables %$x$
whose computation %$\Expr(x)$
involve public input variables only. Indeed, if $\vdash \Oo_1\cup\Oo_2:\sid$ is invalid and $\bigcup_{x\in\Oo_1}\Var({\Expr(x)})\subseteq X_p$, then
$\vdash \Oo_2:\sid$ must be invalid, hence $\vdash \Oo_2:\sdd$ is valid.
Therefore, it suffices to consider
all the size-$d$ subsets $\Oo\subseteq X_o\setminus \{x\in X_o\mid \Var(\Expr(x))\subseteq X_p\}$.


Our divide-and-conquer algorithm for proving order-$d$ secure is shown in Algorithm~\ref{alg:DivHOMaRer}.
Taking a program $P$, sets of public ($X_p$), private ($X_k$),  random
($X_r$) and observable $(X_o)$ variables, and the order $d$ as inputs,
it first computes the set $X$ of observable variables whose computation involves either secret or random variables,
and then initializes the set ${\tt InsecureSets}$ which is used to store all leaky observable sets.
Next, it invokes the function {\sf Explorer} with the set
$\{(d,X)\}$. We assume that $|X|\geq d$, otherwise we can directly check whether
$\vdash X:\sdd$ is valid or not using our type system.

The function {\sf Explorer} is more involved.
It takes a set $\mathcal{Y}$ of pairs $(i,\Oo)$ as input which %for which the following three properties are maintained:
satisfies the following three properties: (1) $\sum_{\{(i,\Oo)\in \mathcal{Y}\}} i=d$, (2) $\biguplus\{\Oo\mid (i,\Oo)\in \mathcal{Y}\}=X$,
and (3) $|\Oo|\geq i$ for all $(i,\Oo)\in \mathcal{Y}$.
It aims at proving that for all pairs $(i,\Oo)\in \mathcal{Y}$
and all possible subsets $\Oo_i$ of $\Oo$ of size $i$,
$\bigcup_{(i,\Oo)\in \mathcal{Y}} \Oo_i$ is order-$d$ secure, i.e., $\vdash \bigcup_{(i,\Oo)\in \mathcal{Y}} \Oo_i:\tau_{\sid}$ is valid.
{\sf Explorer} works as follows.

%=========================================================================================================
\begin{algorithm}[t]
\SetAlgoNoLine
\SetKwProg{myfunc}{Function}{}{}
\myfunc{{\sf HOMV}$(P,X_p,X_k,X_r,X_o,d)$}{
    $X:=\{x\in X_o\mid \Var(\Expr(x))\not\subseteq X_p\}$\;
    ${\tt InsecureSets}:=\emptyset$\;
	{\sf Explorer}$(\{(d,X)\})$\;
}
\medskip
\myfunc{{\sf Explorer}$(\mathcal{Y})$}{
    \ForAll{$(i,\Oo)\in \mathcal{Y}$}{
        Choose a subset $\Oo_i\subseteq \Oo$ such that ${|\Oo_i|}=i$\;
    }
    \If{$\vdash \bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i:\sdd$ is valid}{
        ${\tt InsecureSets}:={\tt InsecureSets}\cup \{\bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i\}$\;
    }
    \ElseIf{$\vdash \bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i:\sid$ is valid (without {\sc Sid}$_2$ rule)}{
        \ForAll{$(i,\Oo)\in \mathcal{Y}$}{
            \ForAll{$x\in\Oo\setminus \Oo_i$}
            {
                \If{$\vdash \{x\}\cup \bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i:\sid$ is valid (without {\sc Sid}$_2$ rule)}{
                    $\Oo_i:=\Oo_i\cup\{x\}$\;
                }
            }
        }
    }

    $\mathcal{Y}':=\{(i,\Oo)\in \mathcal{Y} \mid |\Oo|>i\}$\;
    \lIf{$\mathcal{Y}'=\emptyset$}{\Return}
    \ForAll{$(i,\Oo)\in \mathcal{Y}',  0\leq i_j\leq \min(i,|\Oo\setminus\Oo_i|)$ s.t. $\sum_{(i,\Oo)\in \mathcal{Y}'} i_j\neq 0$}{
        {\sf Explorer}$((\mathcal{Y}\setminus\mathcal{Y}')\cup\{(i-i_j,\Oo_i),(i_j,\Oo\setminus\Oo_i) \mid (i,\Oo)\in \mathcal{Y}'\})$\;
    }
}
\caption{A divide\&conquer algorithm for proving order-$d$ secure}
\label{alg:DivHOMaRer}
\end{algorithm}
%============================================================================================================

It first chooses a size-$i$ subset $\Oo_i$ of $\Oo$ for all pairs $(i,\Oo)\in \mathcal{Y}$,
 and checks whether $\vdash \bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i:\sdd$
is valid  (i.e., the observable set $\bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i$ is order-$d$ secure).
If it is valid, then the set $\bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i$ is added into ${\tt InsecureSets}$; otherwise, $\vdash \bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i:\sid$ must be valid.
{\sf Explorer} proceeds depending upon whether $\vdash \bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i:\sid$
can be proved using the rule {\sc Sid}$_2$ (cf.\ Figure~\ref{tab:semrules}).
\begin{itemize}
  \item If it can be proved \emph{without} using the rule {\sc Sid}$_2$,
 we try to add more variables into sets $\Oo_i$'s. Concretely, for each pair $(i,\Oo)\in \mathcal{Y}$ and variable $x\in\Oo\setminus \Oo_i$, we verify whether $\vdash \{x\}\cup\bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i:\sid$
is still valid %or not is verified
without using the rule {\sc Sid}$_2$.
If the observable set $\{x\}\cup \bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i$
is still order-$d$ secure, $x$ is added into $\Oo_i$.
Otherwise, $x$ is not added into $\Oo_i$.

  \item If it is proved by applying the rule {\sc Sid}$_2$,  we will not extend the sets $\Oo_i$'s for efficiency consideration. Indeed, the premises of rules {\sc Sid}$_2$ and {\sc Sdd}$_3$ are very expensive to verify, and the observable set $\{x\}\cup\bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i$ for any variable
  $x\in \bigcup_{(i,\Oo)\in \mathcal{Y}} \Oo\setminus\Oo_i$ has to be verified using the rule {\sc Sid}$_2$ or {\sc Sdd}$_3$.
\end{itemize}
%

%Now, it is already proved
Given that $\vdash \bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i:\sid$ can be derived, %is valid.
to prove that $\bigcup_{(i,\Oo)\in \mathcal{Y}} \Oo_i'$ are order-$d$ secure for all pairs $(i,\Oo)\in \mathcal{Y}$
and all possible size-$i$ subsets $\Oo_i'$ of $\Oo$,
it remains to prove that the observable sets
$\Oo''=\bigcup_{(i,\Oo)\in \mathcal{Y}} \Oo_i'$ are order-$d$ secure %such that there
where there exists at least one
pair $(i,\Oo)\in \mathcal{Y}$ such that $\Oo'_i$ contains at least two elements from $\Oo\setminus \Oo_i$ and $\Oo_i$ respectively.
%
%some elements (at least one) of $\Oo_i'$ are taking from $\Oo\setminus \Oo_i$
%and some elements (at least one) of $\Oo_i'$ are taken from $\Oo_i$,
%
(Otherwise $\Oo''\subseteq \bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i$).
This is verified by partitioning all the pairs $(i,\Oo)\in \mathcal{Y}$ such that $|\Oo|>i$ into pairs $(i-i_j,\Oo_i),(i_j,\Oo\setminus\Oo_i)$
for all combination of values $0\leq i_j\leq \min(i,|\Oo\setminus\Oo_i|)$ such that
$\sum_{(i,\Oo)\in \mathcal{Y}'} i_j\neq 0$. The condition $\sum_{(i,\Oo)\in \mathcal{Y}'} i_j\neq 0$ is used to avoid the case $\Oo''\subseteq \bigcup_{(i,\Oo)\in \mathcal{Y}}\Oo_i$.
For each combination of values $0\leq i_j\leq \min(i,|\Oo\setminus\Oo_i|)$ such that
$\sum_{(i,\Oo)\in \mathcal{Y}'} i_j\neq 0$, the partitioned pairs $\{(i-i_j,\Oo_i),(i_j,\Oo\setminus\Oo_i) \mid (i,\Oo)\in \mathcal{Y}'\}$ together with the pairs $\{(i,\Oo)\in \mathcal{Y} \mid {|\Oo|}=i\}$
are checked by recursively calling the function {\sf Explorer}.

The procedure terminates as we only partition pairs $(i,\Oo)\in \mathcal{Y}$ such that $|\Oo|>i$
and the sizes of $\Oo_i$ and $\Oo\setminus\Oo_i$ in partitioned pairs $(i-i_j,\Oo_i)$ and $(i_j,\Oo\setminus\Oo_i)$
eventually become smaller and smaller in recursive calls until ${|\Oo|}=i$ or $i=0$.
(Remark that we keep pairs of the form $(0,\Oo)$ into the worklist for simplifying presentation.
They are indeed removed in our implementation.)

\begin{theorem}
The program $P$ is order-$d$ secure iff ${\tt InsecureSets}=\emptyset$.
Moreover, if $P$ is not order-$d$ secure, then ${\tt InsecureSets}$ exactly contains all the possible
size-$d$ observable sets $\Oo\subseteq X_o$ such that $P$ is $\Oo$-leaky.
\end{theorem}

\paragraph{Comparison with the worklist algorithm~\cite{BBDFGS15}.}
%Barthe et al. proposed
A worklist-based space-splitting algorithm for proving order-$d$ secure was proposed in~\cite{BBDFGS15}
which can significantly outperforms both naive enumeration and the pairwise space-splitting algorithm.
Our algorithm is inspired by this algorithm with two key differences.
(1) We introduce model-counting based type inference rules which provide
completeness guarantees, while the algorithm~\cite{BBDFGS15} is incomplete.
(2) The algorithm~\cite{BBDFGS15} appears to have two issues. The first (minor) issue may result in infinite recursion, which
%We remark that this
has been corrected in Algorithm 11, Line 3 of \cite{BBDFGSZ16}. %by some same authors.
The second (and more serious) issue may %result in un
affect soundness.
Indeed, %it may miss out on the checking of
some sets of observable variables might be missed when $d>1$.
%the order $d$ is greater than $1$.
Detailed analysis is given in Appendix~\ref{sec:anaworklistalg}.


   %
%%=====================================================================================================
%\begin{algorithm}[t]
%\SetAlgoNoLine
%\SetKwProg{myfunc}{Function}{}{}
%\myfunc{{\sc Disjoint}$(\Oo)$}{
%    $W:=\emptyset$\;
%    \ForEach{$y\in\Oo$}
%    {
%        \lIf{$\RVar(\Expr(y))\neq\emptyset\wedge\RVar(\Expr(y))\cap W\neq\emptyset$}{ \Return{$\emptyset$}}
%        \lElse{$W:=W\cup \RVar(\Expr(y))$}
%    }
%    \Return{$W$}\;
%}
%\caption{An algorithm for checking disjointness}
%\label{alg:disjoint}
%\end{algorithm}
%%=====================================================================================================
%
%Let us fix $\Oo_1=\{y_1,\cdots,y_m\}$ such that $\vdash y_j:\sid$ for  $1\leq j\leq m$ and
%$\Oo_2=\{x_1,\cdots,x_h\}$ such that $\vdash x_j:\rud$ for $1\leq j\leq h$.
%To check whether $\RVar(\Expr(y_i))\cap \RVar(\Expr(y_j))=\emptyset$  for all $1\leq i\neq j\leq m$,
%we invoke the function {\sc Disjoint}$(\Oo_1)$ in Algorithm~\ref{alg:disjoint}. If
%it returns $\emptyset$, then it does not hold, otherwise it returns the set of variables $W=\bigcup_{j=1}^m\RVar(\Expr(y_j))$.
%
%To check whether
%\[\exists z_1\in \Dom(\Expr(x_1))\setminus \bigcup_{i=1}^m \RVar(\Expr(y_i)),\cdots, \exists z_h\in \Dom(\Expr(x_h))\setminus\bigcup_{i=1}^m \RVar(\Expr(y_i))\]
%with $1\leq i\neq j\leq n. z_i\neq z_j$ holds, we define the predicate
%$\Phi^{\Oo_1\uplus\Oo_2}_W = $ %(recall $\Oo_2=\{x_1, \cdots, x_h\}$) as the following logical formula:
%%
%\[\exists z_1, \cdots, z_h. \left( (\bigwedge_{i=1}^h z_i\in T_i)\wedge {\sf distinct}(z_1,\cdots,z_h)\wedge (\bigwedge_{i=1}^h z_i\not\in W) \right)\]
%where $W=\bigcup_{j=1}^m\RVar(\Expr(y_j))$, $h=|\Oo_2|$, $T_i:=\Dom(\Expr(x_i))$ for $1\leq i\leq h$, and the predicate ${\sf distinct}(z_1,\cdots,z_h)$ asserting that elements from  $(z_1,\cdots,z_h)$ are distinct. %, and $W={\sc Disjoint}(\Oo_1))$.
%
%Using these new predicates, rule {\sc Cp-Sid} can be reformulated as
%\[\inference{\vdash y_1:\sid,  \cdots,  \vdash y_m:\sid & \vdash x_1:\rud,  \cdots, \vdash x_h:\rud \\
%(\exists i:1\leq i\leq m. \RVar(\Expr(y_i))\neq\emptyset)\rightarrow \mbox{{\sc Disjoint}}(\{y_1,\cdots,y_m\})\neq\emptyset \\
% \Phi^{\{x_1,\cdots,x_h\}\uplus\{y_1,\cdots,y_m\}}_{\mbox{{\sc Disjoint}}(\{y_1,\cdots,y_m\})} \ \mbox{is satisfiable} %\mbox{is satisfiable}
%}
%{\vdash \{x_1,\cdots,x_h,y_1,\cdots,y_m\}:\sid}[({\sc Cp-Sid})]\]
%
%Readers may wonder why this (almost trivial) rewriting is interesting. One of the advantages of the new rule is that with the new formulation, it is convenient to verify the premise incrementally by varying $\Oo_1$ or $\Oo_2$. To see this, we can formulate the following three rules:
%%This idea is formalized by the following two new rules:
%\[\begin{array}{r}
%\inference{ \vdash \{x_1,\cdots,x_h,y_1,\cdots,y_m\}:\sid & \vdash y_{m+1}:\sid \\ \RVar(\Expr(y_{m+1}))=\emptyset}{\vdash \{x_1,\cdots,x_h,y_1,\cdots,y_m, y_{m+1}\}:\sid}[({\sc Cp-Extend}$_1$)]\\ \\
%
%\inference{ \vdash \{x_1,\cdots,x_h,y_1,\cdots,y_m\}:\sid & \vdash y_{m+1}:\sid \\ W\neq\emptyset \rightarrow  W\cap \RVar(\Expr(y_{m+1}))\neq\emptyset \\
% \Phi^{\{x_1,\cdots,x_h\}\uplus\{y_1,\cdots,y_m\}}_{W\cup \RVar(\Expr(y_{m+1}))} \mbox{is satisfiable} }{\vdash \{x_1,\cdots,x_h,y_1,\cdots,y_m, y_{m+1}\}:\sid}[({\sc Cp-Extend}$_2$)]\\ \\
%%
%\inference{ \vdash \{x_1,\cdots,x_h,y_1,\cdots,y_m\}:\sid & \vdash x_{h+1}:\rud  \\ \Phi^{\{x_1,\cdots,x_h\}\uplus\{y_1,\cdots,y_m\}}_{W}\wedge\Phi^{x_{h+1}}_{\sf new} \ \mbox{is satisfiable} }{\vdash \{x_1,\cdots,x_h,x_{h+1},y_1,\cdots,y_m\}:\sid}[({\sc Cp-Extend}$_3$)]
%\end{array}\]
%where $W$ denotes the result of $\mbox{{\sc Disjoint}}(\{y_1,\cdots,y_m\})$
%and $\Phi^{x_{h+1}}_{\sf new}$ denotes $\exists z. (z\in\Dom(\Expr(x_{h+1}))\wedge z\not\in W \wedge {\sf distinct}(z_1,\cdots,z_h,z))$.
%
%In rule ({\sc Cp-Extend}$_1$), it suffices to check whether $\vdash \{x_1,\cdots,x_h,y_1,\cdots,y_m\}:\sid$ and $\RVar(\Expr(y_{m+1}))=\emptyset$ hold or not.
%%
%The premises $\Phi^{\{x_1,\cdots,x_h\}\uplus\{y_1,\cdots,y_m\}}_{W\cup \RVar(\Expr(y_{m+1}))}$  and  $\Phi^{\{x_1,\cdots,x_h\}\uplus\{y_1,\cdots,y_m\}}_{W}\wedge\Phi^{x_{h+1}}_{\sf new}$ in rules ({\sc Cp-Extend}$_2$) and ({\sc Cp-Extend}$_3$) can be easily verified using the notion of \emph{scopes}  provided in Z3~\cite{Bjo11}. In general, one may want to explore several similar problems that share several definitions and assertions. Z3 uses the commands \emph{push} and \emph{pop} for this purpose. In a nutshell, Z3 maintains a global stack of declarations and assertions. The command push creates a new scope by saving the current stack size, and pop removes any assertion or declaration performed between it and the matching push.
%%The check-sat and get-assertions commands always operate on the content of the global stack.
%%
%%which provides push and pop commands, where the pop command removes
%%any assertion or declaration performed between the pop and the matching push, while the solver can reuse lemmas learned
%%before the push command.
%
%More concretely, before checking the premises of rules ({\sc Cp-Extend}$_2$) and ({\sc Cp-Extend}$_3$),
%we can perform a push, then add new constraints into the solver. If it succeeds, then we continue to extend other observable variables. Otherwise, it fails to prove in which case we can perform a pop and then try other observable variables. We remark that this algorithm  could be used as a better option for implementing the \textbf{choose} and \textbf{extend} algorithms in~\cite{BBDFGS15}, which are the main barriers of performance in the type system therein.


==> inference_alg.tex <==
%\section{Inference Algorithms}
\section{Efficient Type Inference Algorithms}
\label{sec:3proc}
Our central question is to infer the distribution types of all the subsets $\Oo\subseteq X_o$ of observable variables with size up to $d$ \emph{efficiently}.
%
By examining the premises of type inference rules given in Section~\ref{sec:typesystem}, we identify the following two questions. % to efficiently infer types of a given program.
\begin{description}
  \item[Q1:] How to check whether $\Omega^\Oo$ (cf. Figure~\ref{eq:omega}) is satisfiable? % for rules {\sc Sdd}$_3$ and {\sc Sid}$_2$?
  \item[Q2:] How to %cope with the combinatorial explosion problem? As simply
  avoid naive enumeration of all $\Oo\subseteq X_o$ with $|\Oo|\leq d$, as such a strategy becomes intractable when $d$ and the size of $X_o$ grow.
\end{description}
Neither of these problems can be easily solved using solo syntactic information of the program only. In this section we shall present our solutions.

%In this section, we first discuss algorithms to solve {\bf Q1},
%then present a divide-and-conquer algorithm to handle {\bf Q2}. We will also present %a sound and complete
%transformations which could facilitate  both solutions. %algorithms for both questions.
%which will serve as ingredients of the inference algorithm.  %to efficiently solve the above three challenges and then present
% will be integrated into an overall type inference algorithm in Section~\ref{sec:InferAlg}. %, together with a search strategy over subsets of observable variables, to give the overall type inference algorithm.  \tl{not very sat by my writing, tbi}
%for automatically inferring types of a given program.

%\input{exprsimplify} % do not care variables
\input{smt-based} %smt

%\input{finite-set-constraint} %cp-sid


%\begin{example}
%Consider two observable variables $x_1$ and $x_2$ taking from the implementation of the conversion from second-order Boolean
%to arithmetic masking~\cite{Coron17}, where
%$\Expr(x_1)=(((   (((r_8\oplus r_1)\oplus(((k\oplus r_8)\oplus r_5)\oplus r_3)) - (((k\oplus r_8)\oplus r_5)\oplus r_3))     \oplus r_7  )
%\oplus(((((r_8\oplus r_1)\oplus(((0x0\oplus r_1)\oplus r_2)\oplus r_3))- (((0x0\oplus r_1)\oplus r_2)\oplus r_3)) \oplus r_6) \oplus r_7)) \oplus r_4$,
%$\Expr(x_2)=(((0xFE\odot(r_8\oplus r_1))\oplus (((r_8\oplus r_1)\oplus(r_5\oplus r_2))-(r_5\oplus r_2)))\oplus r_6) \oplus r_4$,
%$k$ is a private input variables, and $r_1-r_8$ are random variables.
%
%
%$\overline{\Expr(x_1)}=(((r_1\oplus((k\oplus r_5)\oplus r_3))-(((k\oplus r_8)\oplus r_5)\oplus r_3))\oplus (((r_8\oplus(r_2\oplus r_3))-((r_1\oplus r_2)\oplus r_3))\oplus r_6)  )\oplus r_4$ and
%$\overline{\Expr(x_2)}=(((0xFE \odot(r_8\oplus r_1)) \oplus(((r_8\oplus r_1)\oplus(r_5\oplus r_2))-(r_5\oplus r_2)))\oplus r_6)\oplus r_4$.
%
%
%need counting
%\end{example}

%\begin{example}
%	Consider $y_2$ in the program in Section~\ref{sec:goubinexample} after inserting presharing,
%	where $\Expr(y_2)=((k\oplus r) \oplus r'-r') \oplus (k\oplus r)$.
%	By Definition~\ref{def:domr}, $k\oplus r$ is dominated by $r$. After replacing  $(k\oplus r)$  with $r$, we get
%	that $\overline{\Expr(y_2)}=(r\oplus r'-r') \oplus r$, which
%	allows us to deduce $\vdash y_2:\sid$ by rule ({\sc Sid}$_0$) (without SMT solving!).
%	This transformation also allows us to reduce the size of SMT formulae, e.g., for sets $\{y_0,y_2\}$ and $\{y_1,y_2\}$.
%\end{example}
%\tl{do we introduce another example?}

%
%Let $\overline{\Psi}^\Oo$ be the SMT formula constructed as $\Psi^\Oo$, but using
%%in which for each variable $x_j\in \Oo$, the expression
%$\overline{e_j}$ instead of $e_j$.
%
%
%\begin{proposition}\label{prop:cut}
%	$\Psi^\Oo$ is satisfiable iff $\overline{\Psi}^\Oo$ is satisfiable.
%\end{proposition}
%
%%\tl{shall we use the text from cav?}
%%The main observation is that: if $e$ is dominated by $r$,
%%then for %every assignment $x\leftarrow e$, the program
%%$\Expr(x)=e$ the program is $x$-uniform. Since we assume that $r$ does not occur in $\{e_1,...,e_m\}$ except $e$,
%%$e$ can be %seen as a \emph{fresh}
%%simply replaced by $r$ when analyzing $\{e_1,...,e_m\}$. Therefore, $\Psi^\Oo$ is satisfiable iff $\overline{\Psi}^\Oo$  is satisfiable.
%
%\begin{corollary}\label{coro:omega2smt}
%	$\Omega^\Oo$ is satisfiable iff $\overline{\Psi}^\Oo$  is satisfiable.
%\end{corollary}

%===========================================================================================================
% the following is the original version

%\paragraph{Dominated Subexpression Elimination}
%As mentioned, the size of $\Psi^\Oo$ is exponential in the number of bits of random variables, so it is crucial to reduce the number of random variables. For this purpose, we propose an approach
%by eliminating dominated sub-expressions.
%Let us fix an observation set $\Oo=\{x_1,\cdots,x_m\}$ with $\Expr(x_1)=e_1,\cdots,\Expr(x_m)=e_m$.

%
%\noindent
%{\bf Dominated Subexpression Elimination}.
%As mentioned, the size of $\Psi^\Oo$ is exponential in the number of bits of random variables, so it is crucial to reduce the number of random variables. For this purpose, we propose an approach
%by eliminating dominated sub-expressions.
%Let us fix an observation set $\Oo=\{x_1,\cdots,x_m\}$ with $\Expr(x_1)=e_1,\cdots,\Expr(x_m)=e_m$.
%
%A sub-expression $e$ in $\Oo$ is \emph{dominated by a random variable $r$}
%if $r\in\Dom(e)$ and $r$ does not occur in $\{e_1,...,e_m\}$ elsewhere.
%$e$ is a \emph{maximally} dominated sub-expression in $\{e_1,...,e_m\}$ if there
%is no other dominated sub-expression $e'$ in $\Oo$ such that $e$ is a (syntactic) sub-expression of $e'$.
%We can observe that $e$ can be simply substituted by some $r\in \Dom(e)$ when analyzing $\{e_1,...,e_m\}$.
%
%A set of variables $Z\subseteq X$ in $\Oo$ is \emph{collapsible} with respect to $\{e_1, \cdots, e_m\}$
%if (1) $Z\subseteq X_p$ or $Z\subseteq X_k$ or $Z\subseteq X_r$,
%and (2) there exist subexpressions $e_1',\cdots, e_k'$ in $\{e_1,...,e_m\}$
%such that for all $1\leq j\leq k$, (i) each variable $z\in Z$ occurs in $e_j'$ exactly once and
%%does not occur in $\{e_1,...,e_m\}$ excluding
%only occurs in $e_1',\cdots, e_k'$,
%and (ii) $e_j'$ can be rewritten as $(\bigoplus_{z\in Z}z)\oplus e_j''$
%%by
%modulo commutativity and associativity of $\oplus$.
%
%It is not difficult to observe that, when $Z$ is collapsible, it can be substituted by %some $z\in Z$
%a fresh variable when analyzing $\{e_1,...,e_m\}$.
%
%Let $\{\overline{e_1},...,\overline{e_m}\}$ denote the set of expressions obtained from $\{e_1,...,e_m\}$
%by: (1) replacing maximally $r$-dominated sub-expression $e$ by $r$ and, (2) replacing collapsible variables $Z$ by some $z\in Z$ \tl{I think this kind of "trick" is confusing, just say a fresh variable respecting the type}.
%Let $\overline{\Psi}^\Oo$ be the SMT formula constructed as $\Psi^\Oo$, but using
%%in which for each variable $x_j\in \Oo$, the expression
%$\overline{e_j}$ instead of $e_j$.
%
%
%\begin{proposition}\label{prop:cut}
%$\Psi^\Oo$ is satisfiable iff $\overline{\Psi}^\Oo$ is satisfiable.
%\end{proposition}
%
%%\tl{shall we use the text from cav?}
%%The main observation is that: if $e$ is dominated by $r$,
%%then for %every assignment $x\leftarrow e$, the program
%%$\Expr(x)=e$ the program is $x$-uniform. Since we assume that $r$ does not occur in $\{e_1,...,e_m\}$ except $e$,
%%$e$ can be %seen as a \emph{fresh}
%%simply replaced by $r$ when analyzing $\{e_1,...,e_m\}$. Therefore, $\Psi^\Oo$ is satisfiable iff $\overline{\Psi}^\Oo$  is satisfiable.
%
%\begin{corollary}\label{coro:omega2smt}
%$\Omega^\Oo$ is satisfiable iff $\overline{\Psi}^\Oo$  is satisfiable.
%\end{corollary}
%
%\begin{example}
%Consider $y_2$ in the program in Section~\ref{sec:goubinexample} after inserting presharing,
%where $\Expr(y_2)=((k\oplus r) \oplus r'-r') \oplus (k\oplus r)$.
%Then $k\oplus r$ is dominated by $r$. After replacing  $(k\oplus r)$  with $r$, we get
%that $\overline{\Expr(y_2)}=(r\oplus r'-r') \oplus r$, which
%allow us to deduce $\vdash y_2:\sid$ by rule ({\sc Sid}$_0$) even without SMT solving.
%This also allows us to reduce the size of SMT formulae, e.g., for sets $\{y_0,y_2\}$ and $\{y_1,y_2\}$.
%\end{example}


%
%
%\[\begin{array}{ll}
%  \Expr(y_0)=(k\oplus r) \oplus r'; &
%  \Expr(y_1)=(k\oplus r) \oplus r'-r'; \\
%  \Expr(y_2)=((k\oplus r) \oplus r'-r') \oplus (k\oplus r); ~~~~~~~~~~~~&
%  \Expr(y_3)=r' \oplus r; \\
%  \Expr(y_4)=(r'\oplus r)\oplus (k\oplus r) &
%  \Expr(y_5)=((r'\oplus r)\oplus (k\oplus r))- (r' \oplus r); \\
%  \multicolumn{2}{l}{\Expr(A)=(((r'\oplus r)\oplus (k\oplus r))- (r' \oplus r)) \oplus  (((k\oplus r) \oplus r'-r') \oplus (k\oplus r)); }
%\end{array}\]
%
%
%
%
%%======================================================================
%\section{Type Inference Algorithms}\label{sec:InferAlg}
%%====================================================================
%
%%We now describe a simple algorithm for soundly and completely checking whether a program
%%$P$ is order-$d$ probing secure or not.
%
%In this section, we present a type inference algorithm based on the procedures given in the previous section. Let us fix a program $P$ with public ($X_p$), private ($X_k$),  random
%($X_r$) and observable $(X_o)$ variables.
%%
%We shall extend the approach %the type inference for each variable the algorithmic contribution
%of Zhang et al. \cite{ZGSW18} that supports %a refinement based type inference for
%proving \emph{first-order} probing secure of \emph{Boolean programs} only. There are several challenges to overcome.
%%even proving that a program is first-order probing secure can be handled in a relatively efficient way.
%%algorithm to  proving a program is order-$d$ probing secure remains a complex task: indeed this involves
%In particular, for order-$d$ probing secure one needs to infer types of all subsets $\Oo\subseteq X_o$ with size $d$, which easily leads to combinatorial explosion for large $d$. We first present a simple algorithm %for proving order-$d$ probing secure
%by enumerating all possible such subsets, but then present a divide and conquer algorithm aiming to avoid the naive brutal force enumeration. %check all the possible combinations.
%%
%The algorithm presented here will invoke a procedure ${\sf MaRer}(\cdot)$ from \cite{ZGSW18} to type individual observable variables (i.e., to handle the first-order masking). However, here we improve and extend the original version of ${\sf MaRer}(\cdot)$ by (1) an improved approach to compute $\RVar(x)$,
%(2) an SMT-based approach to simplify expression $e$, and (3) addressing arithmetic programs in addition to Boolean programs.
%
%
%%%actually improves the procedure in \cite{ZGSW18}
%%by (1) an improved approach to compute $\RVar(x)$,
%%(2) the SMT based approach is applied on the simplified expression $\widehat{e}$,
%%(3) addressing \emph{higher-order masking} of \emph{Arithmetic programs} rather than \emph{first-order} of \emph{Boolean programs}.
%%%(3) target algorithm for first-order to higher-order.%  \tl{anything else? please improve this}
%%%These changes make to tool significantly fast to infer types of all variables.
%
%%================I commented out, but may need some material later=================
%
%%\tl{will see whether this paragraph is needed}
%%Their work takes a program as input and represents the
%%program as a data dependency graph (that is a directed acyclic graph), traverses the graph in a topological order from leaf to root
%%to infer a type for each observable variable.
%%During inferring the type of a variable $x$, it first uses a less precise set $\RVar(\Expr(x))$ instead of $\RVar(x)$.
%%If it fails to infer the type using $\RVar(\Expr(x))$, then uses a more accurate set $\RVar(x)$.
%%The type system is still sound by replacing $\RVar(\Expr(x))$ with $\RVar(x)$, as $\RVar(\Expr(x))\subseteq\RVar(x)$.
%%Moreover, $\RVar(\Expr(x))$ can be computed in linear time, which is more easy than computing $\RVar(x)$.
%%Finally, the SMT based approach introduced by Eldib et al.~\cite{EWS14b} is used to determine the type of $x$ if it fails to infer the type of $x$ using $\RVar(x)$.
%%
%%\tl{what is the point here?}
%%We adapt their algorithms by changing the $\RVar(x)$ computing in one way.
%%We compute $\RVar(x)$ by invoking our algorithm (Algorithm~\ref{alg:usage}) instead of naively computing $\RVar(x)$
%%by checking each random variable. Moreover, the SMT based approach is applied on the simplified expression $\widehat{e}$.
%%These changes make to tool significantly fast to infer types of all variables.
%%We denote by function {\sf MaRer}$(P)$ the optimized algorithm for inferring types of all the variables $X_o$ of $P$.
%%=======================================================================================
%
%\subsection{A Simple Algorithm}
%\begin{algorithm}[h]
%\SetAlgoNoLine
%\SetKwProg{myfunc}{Function}{}{}
%\myfunc{{\sf HOMaRer}$(P,X_o,d)$}{
%    {\sf MaRer}$(P)$\;
%    \ForAll{$\Oo\subseteq X_o\wedge {|\Oo|}=d$}{
%          {\sf Check}$(\Oo)$\;
%    }
%}
%\medskip
%\myfunc{{\sf Check}$(\Oo)$}{
%      \If{$\exists x\in\Oo.\vdash x:\sdd$}{$\vdash \Oo:\sdd$ (Rule {\sc Cp-Sdd})\;}
%      \ForAll{$x\in \Oo$}{$\Expr(x):=${\sf Simplify}$(\Expr(x))$\;}
%      \If{$X_k\cap\bigcup_{x\in\Oo}\Var( \overline{\Expr(x)})=\emptyset$}{$\vdash \Oo:\sid$ (Rule {\sc Cp-Ind})\;}
%      \ElseIf{{\tt Premises of rule ({\sc Cp-Sid}) hold on $\Oo$ with $(\overline{\Expr(x)})_{x\in\Oo}$}}{$\vdash \Oo:\sid$ (Rule {\sc Cp-Sid})\;}
%      \ElseIf{$\overline{\Psi}^\Oo$ {\tt is satisfiable}}{$\vdash \Oo:\sdd$ (Rule {\sc Sdd}$_3$)\;}
%      \lElse{$\vdash \Oo:\sid$ (Rule {\sc Sid}$_2$)}
%}
%\caption{A simple algorithm for proving order-$d$ probing secure}
%\label{alg:HOMaRer}
%\end{algorithm}
%
%
%Our simple algorithm %for proving order-$d$ probing secure
%is shown in Algorithm~\ref{alg:HOMaRer}.
%It first uses the function {\sf MaRer}$(P)$ to infer the types of all the observable variables $X_o$, so the first-order case can be solved.
%Then, for each possible set $\Oo\subseteq X_o$ with size $d$,
%it iteratively  applies rules ({\sc Cp-Sdd}), ({\sc Cp-Ind}), ({\sc Cp-Sid}), ({\sc Sdd}$_3$) and ({\sc Sid}$_2$). Note that the order reflects the complexity of applying respective rules.
%
%Recall that the size of $\overline{\Psi}^\Oo$ is exponential in the number of bits of random variables and the satisfiability problem
%of $\overline{\Psi}^\Oo$ is intractable. To mitigate this issue, before applying the SMT solver to $\overline{\Psi}^\Oo$,
%we first check $\overline{\Psi}^\Oo$ by verifying whether $\sem{P}^\Oo_{\eta_1}=\sem{P}^\Oo_{\eta_2}$ for some specific valuations $(\eta_1,\eta_2)\in \Theta^2_{=X_p}$.
%This allows us to quickly identify flaws without the heavy SMT solving.
%
%%in the order of their computational complexities.
%%
%%More technically, we provide two algorithms: {\sf ReCombGen} and {\sf NonReCombGen}, for recursive and non-recursive enumerating combinations $\Oo$ from $X_o$.
%%{\sf ReCombGen} is a classic recursive algorithm for generating combinations.
%%{\sf NonReCombGen} is an adjacent interchange generation of combinations from~\cite{Rus88}.
%%In general, {\sf ReCombGen} has better complexity than {\sf NonReCombGen}, as the latter
%%has to search backward adjacent interchangeable positions,
%%However, {\sf ReCombGen} may cause a stack overflow. Therefore, we implement
%%both algorithms. The pseudo code of algorithms {\sf ReCombGen} and {\sf NonReCombGen} are given Appendix~\ref{sec:algcom}.
%
%
%\begin{theorem}\label{thm:HOMaRerSimple}
%The program $P$ is order-$d$ probing secure iff Algorithm~\ref{alg:HOMaRer} does not produce $\vdash \Oo:\sdd$.
%\end{theorem}
%
%%===========================
%%
%%===========================
%
%\subsection{A More Efficient Search Strategy}
%
%Exhaustive enumeration of all subsets of observable variables  may not scale %quickly become intractable
%when $d$ and $X_o$ grow. We then present a divide-and-conquer algorithm %for verifying order-$d$ probing secure,
%inspired by the prior work of Barthe at al.~\cite{BBDFGS15}. Recall the following simple observations.
%\begin{description}
%	\item[Observation 1:]  If $\vdash \Oo:\sid$ is valid, then $\vdash \Oo':\sid$ is valid for all $\Oo'\subseteq \Oo$ (cf. Proposition~\ref{prop:uniform2SI}(ii)).
%	\item[Observation 2:]  If $\vdash x:\sdd$ is valid, then $\vdash \Oo:\sdd$ is valid for all $\Oo\subseteq X_o$ with $x\in \Oo$, i.e., rule ({\sc Cp-Sdd}) in Figure~\ref{tab:semrules}.
%	\item[Observation 3:]  If $X_k\cap\bigcup_{x\in\Oo}\Var({\Expr(x)})=\emptyset$, then $\vdash \Oo:\sid$ is valid, i.e., rule ({\sc Cp-Ind}) in Figure~\ref{tab:semrules}.
%\end{description}
%



==> smt-based.tex <==
\subsection{Q1: Checking Satisfiability of $\Omega^\Oo$}\label{sec:smt}

Fix a set of observable variables $\Oo=\{x_1,\cdots,x_m\}$. Recall the equation \eqref{eq:omega}.\\
$\Omega^\Oo\equiv\exists (\eta_1,\eta_2)\in \Theta^2_{=X_p}.\exists (c_1,\cdots,c_m)\in\Bb^m.
(\sharp_{\eta_1}(c_1,\cdots,c_m)\neq\sharp_{\eta_2}(c_1,\cdots,c_m)).$\\
%where $\sharp_{\eta}(c_1,\cdots,c_m)$ denotes the number of valuations $\eta_r:X_r\rightarrow\Bb$ such that
%for all $j:1\leq j\leq m$: $c_j=\Expr_{\eta,\eta_r}(x_j)$,  and $\Expr_{\eta,\eta_r}(x_j)$ denotes
%expression obtained from $\Expr_{\eta}(x_j)$ by replacing each occurrence of a variable $y\in X_r$ with its value $\eta_r(y)$.
%
%$\Omega^\Oo$ is a model-counting constraint, and %no efficient solution exists  as
%the model-counting problem of propositional formulae is known to be $\sharp P$-hard.
%In this subsection,
We shall discuss two approaches for checking the satisfiability of
$\Omega^\Oo$: an SMT-based approach and a brute-force approach with possibly GPU acceleration.
%and a GPU accelerated brute-force approach.

\medskip
\noindent\emph{SMT-based approach.}
The SMT-based approaches were proposed for checking satisfiability of
$\Omega^\Oo$ for \emph{first-order} Boolean programs~\cite{EWS14b,ZGSW18} and arithmetic programs~\cite{GXZSC19}.
The main idea is to reduce the satisfiability problem of $\Omega^\Oo$ to the satisfiability problem of a (quantified-free) first-order logic formula that can be solved by SMT solvers.
%Therefore, the first approach that come into mind to solve the question {\bf Q1} is to
It would be natural to generalise the SMT-encoding  for first-order \cite{GXZSC19} to higher-order.
In Appendix~\ref{sec:smt-encoding}, we give the formal SMT-encoding (with an example), which appears to the best way to  encode the satisfiability of $\Omega^\Oo$ in SMT formula.
%To our knowledge, it is the best way to
This approach is feasible, but according to our experiments, is practically unfavourable because of its poor scalability. %in terms of performance, as the size of the SMT formula is exponential in the number of
%bits of random variables.
Indeed, it is shown in~\cite{GXZSC19} that for the first-order case,
%the SMT-based approach is comparable to a brute-force approach
%on Boolean programs, but the latter approach significantly
this approach is defeated %outperforms
by a brute-force approach for a majority of arithmetic program benchmarks.  %(except for one benchmark).
%Therefore, an alternative approach is to extend the brute-force approach of~\cite{GXZSC19} from first-order to higher-order.

\medskip
\noindent\emph{Brute-force approach.}
The brute-force approach (cf. Algorithm~\ref{alg:bfalg}) enumerates all possible valuations %$\sigma$
and then computes corresponding distributions %$\sem{x}_{\sigma}$  %for each pair $(\sigma,\sigma_2)$
again by enumerating the assignments of random variables.
%------------------------- no space for this --------------------------------
%Algorithm~\ref{alg:bfalg} gives the pseudo-code.
%It iteratively enumerates valuations $\eta_p$ of public input variables.
%For each enumeration $\eta_p$, Algorithm~\ref{alg:bfalg} then iteratively enumerates
%valuations $\eta_k$ of secret input variables.
%Next, it invokes the {\sc Counting} function to compute the distribution of
%$\sem{P}^\Oo_{\eta_p,\eta_k}$ by enumerating all the possible valuations of
%random variables, the result is stored in the array $D_1$ for the first enumeration of secret input variables or $D_2$
%for the other enumeration of secret input variables.
%Finally, it compares whether $D_1$ or $D_2$ are same or not.
%If they are not same, we get that $\Omega^\Oo$ is satisfiable. Otherwise, it continues
%the enumeration.
%---------------------------------------------------------------------------------------
\begin{algorithm}[t]
\SetAlgoNoLine
\SetKwProg{myfunc}{Function}{}{}
\myfunc{{\sc BFEnum}$(P,\Oo=\{x_1,\cdots,x_m\})$}{
    \ForAll{$\eta_p:\bigcup_{x\in \Oo}X_p\cap \Var(\Expr(x)) \rightarrow \Bb$}{
        $D_1:=\lambda (c_1,\cdots,c_m)\in \Bb^m.0$\;
        $b:={\tt false}$\;
        \ForAll{$\eta_k:\bigcup_{x\in \Oo}X_k\cap \Var(\Expr(x)) \rightarrow \Bb$}{
            $D_2:=\lambda (c_1,\cdots,c_m)\in \Bb^m.0$\;
            \If{$b={\tt false}$}{
                $D_1:=${\sc Counting}$(P,\Oo,\eta_p,\eta_k)$\;
                $b:={\tt true}$\;
            }
            \Else{
                $D_2:=${\sc Counting}$(P,\Oo,\eta_p,\eta_k)$\;
                \If{$D_1\neq D_2$}{\Return{${\tt SAT}$}\;}
            }
        }
    }
    \Return{${\tt UNSAT}$}\;
}
\medskip
\myfunc{{\sc Counting}$(P,\Oo=\{x_1,\cdots,x_m\},\eta_p,\eta_k)$}{
    \ForAll{$\eta_r:\bigcup_{x\in \Oo}\RVar(\Expr(x)) \rightarrow \Bb$}{
        $D[\Expr_{\eta_p,\eta_k,\eta_r}(x_1),\cdots,\Expr_{\eta_p,\eta_k,\eta_r}(x_m)]++$\;
    }
    \Return{$D$}\;
}
\caption{A brute-force algorithm\label{alg:bfalg}}
\end{algorithm}
%---------------------------------------------------------------------------------------------
\begin{lemma}
$\Omega^\Oo$ is satisfiable iff  Algorithm~\ref{alg:bfalg} returns ${\tt SAT}$.
\end{lemma}

The complexity of Algorithm~\ref{alg:bfalg} is exponential in the number of (bits of) variables in $\{\Expr(x)\mid x\in\Oo\}$
%Hence, it would be intractable
so it would experience significant performance degradation when facing a large number of variables.
%if the number variables in $\{\Expr(x)\mid x\in\Oo\}$ is large.
%To accelerate computation,
We propose a GPU-accelerated parallel algorithm to boost the performance. %for checking satisfiability of $\Omega^\Oo$.

\medskip
\noindent\emph{GPU-accelerated parallel algorithm.}
%GPUs have been widely used to accelerate scientific, engineering and industry computations.
Our work is based on CUDA, a parallel computing platform and programming model for NVIDIA GPUs.
%In this work, we
In particular, we utilize Nvidia GeForce GTX 1080 (Pascal) with compute capability 6.1.
%(architecture details refer to its whitepaper~\footnote{NVIDIA GeForce GTX 1080
%whitepaper: \url{https://international.download.nvidia.cn/geforce-com/international/pdfs/GeForce_GTX_1080_Whitepaper_FINAL.pdf}.}).
From a programming perspective,
%\footnote{CUDA C programming guide: \url{https://docs.nvidia.com/cuda/cuda-c-programming-guide}.},
the CUDA architecture defines three levels of threads, i.e., grid, block and warp, to organize units.
A warp consists of 32 consecutive threads %and all threads in a warp
which are executed in the Single Instruction Multiple Thread fashion on Streaming Processors,
namely, all threads execute the same instruction, and each thread carries out that operation on its own private data.
A block running on Streaming Multiprocessors (SM) contains at most $32$ wraps (giving rise to $32\times 32$ threads).
The maximum number of blocks in a grid is $65535\times 65535$ and each grid runs on the Scalable Streaming Processor Array (SPA). The code running on GPUs is usually referred to as Kernel.

We parallelize Algorithm~\ref{alg:bfalg} as a CUDA program. In this work, we focus on byte programs, i.e., each
variable is of 8-bit. %In our experiments, we find that
Typically, the number of random variables is usually much larger than that of the other %input
variables.
Therefore, we  enumerate valuations of random variables in GPUs while enumerate valuations of public and input variables in CPUs. Namely, the {\sc Counting} function in Algorithm~\ref{alg:bfalg} is implemented as a Kernel. However, it would be difficult to implement a generic
Kernel to compute distributions of sets of expressions $\{\Expr(x)\mid x\in\Oo\}$, unless
expressions are evaluated by traversing their parse trees, which is control-flow intensive and would downgrade the GPU performance. As a result, instead of designing a generic Kernel, for each set $\Oo$ of observable variables, we synthesize a CUDA program which checks whether
$\Omega^\Oo$ is satisfiable based on Algorithm~\ref{alg:bfalg}.
%Due to lack of space,
The skeleton of the synthesized GPU programs is given in Appendix~\ref{sec:gpualg}.


The numbers of threads per block and blocks per grid in each synthesized CUDA program are determined
by the number $R:=|\bigcup_{x\in\Oo}\RVar(\Expr(x))|$ of random variables in $\{\Expr(x)\mid x\in\Oo\}$.
If $R=3$, we choose 2-D $(16,16)$ blocks each of which has $2^8$ threads,
and 2-D $(256,256)$ grids each of which has $2^{16}$ blocks. (Note that the number $2^{24}$ of threads exactly corresponds to the number of valuations of
three 8-bits random variables.) Moreover, we do not need to enumerate those valuations,
as the thread Id and block Id (i.e., \textsf{threadIdx} and \textsf{blockIdx} in CUDA) of each host thread in GPU exactly corresponds one of those valuations.
If %the number of random variables is less than
$R<3$, we reduce
the number of blocks and/or threads such that the total number of threads is the number of valuations
of random variables. Otherwise $R>3$, %, if the number of random variables is greater than $3$,
we set $2^8$ number of threads in each block and $2^{16}$ number blocks in one grid for three random variables,
while the valuations of the rest of the random variables are enumerated in GPU.


For each operation used in expressions of $\{\Expr(x)\mid x\in\Oo\}$ but is not supported in CUDA, we synthesize
a corresponding \textsf{\_\_device\_\_} function which will be called from GPUs only and executed therein.
For each expression $\Expr(x)$, we also synthesize a \textsf{\_\_device\_\_} function
which computes the value of the expression using \textsf{\_\_device\_\_} functions for operations based on
thread Id and block Id of the host thread which represent the valuations of some random variables.


%\tl{this para is not self-contained, may be removed later}
%cudaMal-
%locManaged function by which the managed pointer is valid on both the GPU
%and CPU

For memory management, we use int arrays to store distributions, which are accessed both from
CPU for comparing distributions (read-only) and GPU for computing distributions (write-only).
%, and data race should be avoided in parallel computing.
We utilize unified memory provided by CUDA to allocate memory for both int arrays,  %$D_1$ and $D_2$,
namely, to allocate memory by invoking the \textsf{cudaMallocManaged},
by which the managed pointers to int arrays are valid on both the GPU and CPU.
To resolve data race, the update of int arrays in Kernel is performed in one atomic transaction (via the \textsf{atomicAdd} function in CUDA).

%store distributions should be accessed both from
%CPU for comparing distributions (read-only) and GPU for updating distributions (write-only), and data race
%should be avoided in parallel computing.
%We utilize unified memory provided by CUDA to allocate memory for $D_1$ and $D_2$,
%namely allocating memory by invoking the \textsf{cudaMallocManaged},
%by which the managed pointers to $D_1$ and $D_2$ are valid on both the GPU and CPU.
%To avoid data race, the update of $D_1$ and $D_2$ in Kernel is performed in one atomic transaction (the \textsf{atomicAdd} function in CUDA).
%Due to lack of space, the skeleton of synthesized GPU programs is given in Appendix~\ref{sec:gpualg}.




==> worklist-alg.tex <==



\section{The Approach from~\cite{BBDFGS15}}
\label{sec:anaworklistalg}
In this section, we first briefly recall the worklist-based space-splitting (BBDFGS) algorithm from~\cite{BBDFGS15}, which
is currently the most efficient algorithm for proving higher-order security of masked arithmetic programs under the ISW threshold probing model.
Unfortunately, this algorithm suffers from two subtle issues which we will discuss.
More details of BBDFGS refer to~\cite{BBDFGS15}.

\subsection{The Proof System}\label{sec:berthesproofsys}
An expression (i.e., function) $e(x_1,\cdots,x_n)$ is \emph{$i$-invertible} if, for any concrete
values $c_1,\cdots,c_{i-1},c_{i+1},\cdots, c_n\in \Bb$,
the expression
\begin{center}
$e(c_1/x_1,\cdots,c_{i-1}/x_{i-1},x_i,c_{i+1}/x_{i+1},\cdots, c_n/x_{n})$
\end{center}
obtained by instantiating all the variables $(x_j)_{j\neq i}$
with concrete values $(c_j)_{j\neq i}$ is bijective.


%We can show that checking whether
%an expression $e(x_1,\cdots,x_n)$ is $i$-invertible or not is co\textbf{NP}-complete.
%
%\begin{proposition}\label{prop:NPcomplete}
%The $i$-invertibility problem is co\textbf{NP}-complete.
%\end{proposition}
%
%\begin{proof}
%We show that non $i$-invertibility is \textbf{NP}-complete.
%
%\noindent{\bf Upper-bound}.
%Consider an expression $e(x_1,\cdots,x_n)$,
%to prove that
%$e(x_1,\cdots,x_n)$ is not $i$-invertible,
%we can nondeterministically
%guess concrete values $c_1,\cdots,c_{i-1},c_{i+1},\cdots, c_n\in \Bb$
%and two values $c$ and $c'$ for $x_i$ such that $c\neq c'$, and then
%verify whether the values of the following two expressions
%\[\begin{array}{cc}
%  e(c_1/x_1,\cdots,c_{i-1}/x_{i-1},c/x_i,c_{i+1}/x_{i+1},\cdots, c_n/x_{n}) \\
%  e(c_1/x_1,\cdots,c_{i-1}/x_{i-1},c'/x_i,c_{i+1}/x_{i+1},\cdots, c_n/x_{n})
%\end{array}\]
%are identical or not. If the values of these two expressions are identical,
%then $e(c_1/x_1,\cdots,c_{i-1}/x_{i-1},x_i,c_{i+1}/x_{i+1},\cdots, c_n/x_{n})$ is not a bijection, hence
%$e(x_1,\cdots,x_n)$ is not $i$-invertible.
%
%\medskip
%\noindent
%{\bf Lower-bound}.
%We reduce from the 3SAT problem which is known to be \textbf{NP}-complete.
%Consider a Boolean formula $\phi=\bigvee_{i=1}^m(\ell_1^1\wedge \ell_2^1\wedge \ell_3^1)$
%over a set of Boolean variables $\{x_1,\cdots,x_n\}$, $\phi$ is satisfiable iff there exists an assignment $f:\{x_1,\cdots,x_n\}\rightarrow\{0,1\}$
%such that $\phi$ evaluates to $1$ under the assignment $f$.
%Let $e_{b}(x_1',\cdots,x_n')$ be the expression defined as follows:
%\[
%e_b(x_1',\cdots,x_n')=\left\{
%\begin{array}{ll}
%  x_i', & \mbox{if }\exists 1\leq j\leq n: \ x_j'\not\in\{0,1\} \\
%  \phi'\vee (b\neq x_i'), &  \mbox{otherwise.}
%\end{array}
%\right.
%\]
%where $\phi'$ is the Boolean formula obtained from $\phi$ by replacing all the occurrences
%of each variable $x\in \{x_1,\cdots,x_n\}$ by $x'$.
%Remark that $e_{b}(x_1',\cdots,x_n')$ can be transformed into an expression
%in the syntax of our programming language.
%
%\medskip
%\noindent
%{\bf Claim}.  $\phi$ is satisfiable iff either $e_{1}(x_1',\cdots,x_n')$ or $e_{0}(x_1',\cdots,x_n')$ is not $i$-invertible.
%
%\medskip
%\noindent
%{\bf ``If'' direction}.  Suppose that either $e_{1}(x_1',\cdots,x_n')$ or $e_{0}(x_1',\cdots,x_n')$ is not $i$-invertible.
%We prove by contradiction. Suppose $\phi$ is not satisfiable, then $e_{1}(x_1',\cdots,x_n')$ and $e_{0}(x_1',\cdots,x_n')$ can be simplified as:
%\[
%e_0(x_1',\cdots,x_n')=\left\{
%\begin{array}{ll}
%  x_i', & \mbox{if }\exists 1\leq j\leq n: \ x_j'\not\in\{0,1\} \\
%  x_i', &  \mbox{otherwise.}
%\end{array}
%\right.
%\]
% \[
%e_1(x_1',\cdots,x_n')=\left\{
%\begin{array}{ll}
%  x_i', & \mbox{if }\exists 1\leq j\leq n: \ x_j'\not\in\{0,1\} \\
%  1\neq x_i', &  \mbox{otherwise.}
%\end{array}
%\right.
%\]
%We get that
%for all $c_1,\cdots, c_{i-1},c_{i+1},\cdots,c_n\in\Bb$, $b\in\{0,1\}$
%\[e_{b}(c_1/x_1',\cdots,c_{i-1}/x_{i-1}',x_i',c_{i+1}/x'_{i+1},\cdots, c_n/x_n')\]
%is a bijective function. Hence, both $e_0(x_1',\cdots,x_n')$
%and $e_1(x_1',\cdots,x_n')$ are $i$-invertible, which contradicts to the fact that either $e_{1}(x_1',\cdots,x_n')$ or $e_{0}(x_1',\cdots,x_n')$ is not $i$-invertible.
%
%
%\medskip
%\noindent
%{\bf ``Only if'' direction.}
%Suppose $\phi$ is satisfiable under the assignment
%$f:\{x_1,\cdots,x_n\}\rightarrow\{0,1\}$. Let $f':\{x_1,\cdots,x_n\}\rightarrow\{0,1\}$ be the assignment
%such that for every $x\in \{x_1,\cdots,x_n\}$, $f(x)=f'(x)$ if $x\neq x_i$, otherwise
%$f(x)=\neg f'(x)$.
%\begin{itemize}%[topsep=1pt,leftmargin=*]
%  \item If $f(x_i)=1$, then $e_{1}(f(x_1)/x_1',\cdots,f(x_n)/x_n')=1$ and $e_{1}(f'(x_1)/x_1',\cdots,f'(x_n)/x_n')=1$. Hence, $e_{1}(x_1',\cdots,x_n')$ is not $i$-invertible.
%  \item If $f(x_i)=0$, then $e_{0}(f(x_1)/x_1',\cdots,f(x_n)/x_n')=1$ and $e_{0}(f'(x_1)/x_1',\cdots,f'(x_n)/x_n')=1$. Hence, $e_{0}(x_1',\cdots,x_n')$ is not $i$-invertible.
%\end{itemize}
%
%Therefore, either $e_{1}(x_1',\cdots,x_n')$ or $e_{0}(x_1',\cdots,x_n')$ is not $i$-invertible.
%\end{proof}

Given a program $P$ annotated with the public ($X_p$),
private ($X_k$), and random ($X_r$) variables,
the judgments are in the form of $(X_p,X_k) \vdash E$,
where $E$ is a set of expressions.
The judgment $(X_p,X_k) \vdash \{\Expr(x)\mid x\in\Oo\}$ is valid
iff $P$ is $\Oo$-\SI.
Figure~\ref{fig:bartherules} presents the sound proof system of~\cite{BBDFGS15}
for deriving the valid judgments.


\begin{figure}[h]
\centering
\scalebox{0.85}{
\begin{tabular}{rr}
$\inference{\Var(E)\cap X_k=\emptyset}{(X_p,X_k) \vdash E}[{\sc Indep}]$ & $\inference{(X_p,X_k) \vdash E & E=_{ET}E'}{(X_p,X_k) \vdash E'}[{\sc Conv}]$\\
\multicolumn{2}{c}{$\inference{(X_p,X_k) \vdash E & e'(x_1,\cdots,x_n) \text{ is $ i$-invertible} & x_i\in X_r} {(X_p,X_k) \vdash E[e'(x_1,\cdots,x_n) /x_i]}[({\sc Opt})]$}
\end{tabular}}
\caption{Proof system from~\cite{BBDFGS15}.}
\label{fig:bartherules}
\end{figure}

Rule ({\sc Indep}) is straightforward and is similar to our rule ({\sc No-Key}).
Rule ({\sc Conv}) states that if $(X_p,X_k) \vdash E$ is valid, then
$(X_p,X_k) \vdash E'$ is valid for any $E'$ that
is equivalent to $E$ with respect to some provided equational theory $ET$.
Rule ({\sc Opt}) states if $(X_p,X_k) \vdash E$ is valid
and the expression $e'(x_1,\cdots,x_n)$ is $i$-invertible with $x_i$ being a random variable,
then $(X_p,X_k) \vdash E[e'(x_1,\cdots,x_n) /x_i]$ is valid,
where $E[e'(x_1,\cdots,x_n) /x_i]$ denotes the set of expressions obtained by replacing
all the occurrences of $x_i$ in $E$ by $e'(x_1,\cdots,x_n)$.
This rule can be seen as an integration of our transformation  $\simply_{\Dom}(E)$
into the type proof system.

%It is stated in~\cite{BBDFGS15}, ``the first (leftmost-first depth-first) random variable $x_i$
%that fulfills the $i$-invertible condition is selected and then the largest superterm of $x_i$  \tl{what does it mean by largest expression?}
%that fulfills the $i$-invertible condition is selected''.
%However, \cite{BBDFGS15} does not explicitly present any algorithms to verify the $i$-invertible conditions.



Given a set of expressions $E$,
we denote by ${\tt NI}_{X_p,X_k}(E)$ the procedure for proving
whether $(X_p,X_k) \vdash E$ is valid or not using the proof system in Figure~\ref{fig:bartherules}.
${\tt NI}_{X_p,X_k}(E)$ iteratively applies the Rule ({\sc Indep}), Rule ({\sc Opt})
and Rule ({\sc Conv}), where Rule ({\sc Conv}) is applied at most once in~\cite{BBDFGS15} because it is time-consuming.
Finally, it either returns the proof or $\bot$ if it fails to prove.
%
%, until it proves that $(X_p,X_k) \vdash E$ is valid, or . \tl{how to guarantee termination?}
%In the first case, ${\tt NI}_{X_p,X_k}(E)$ , otherwise returns

\subsection{The BBDFGS Algorithm}
\begin{algorithm}[t]
\SetAlgoNoLine
\SetKwProg{myfunc}{Function}{}{}
\myfunc{${\tt check}_{X_p,X_k}((d_j,E_j)_{0\leq j< n})$}{
    \If{$\forall j,d_j\leq |E_j|$}{
        $Y_j\leftarrow {\tt choose}(\mathcal{P}_{\leq d_j}(E_j))$\;
        $\vec{h}\leftarrow {\tt NI}_{X_p,X_k}(\bigcup_{0\leq j< n}Y_j)$\;
        \lIf{$\vec{h}=\bot$} {{raise error CannotProve}$(\bigcup_{j=0}^{n-1}Y_j)$}
        $\widehat{Y_j}\leftarrow {\tt extend}_{X_p,X_k}(Y_j,E_j\setminus Y_j,\vec{h})$\;
        ${\tt check}_{X_p,X_k}((d_j,E_j\setminus \widehat{Y_j})_{0\leq j< n})$\;
        \For{$j; 0<i_j< d_j$}{
            ${\tt check}_{X_p,X_k}((i_j,\widehat{Y_j}), (d_j-i_j,E_j\setminus \widehat{Y_j}))$\;
        }
}
%\tl{need to mention $d_j$?}
}
\caption{The BBDFGS algorithm~\cite{BBDFGS15}}
\label{alg:worklistalg}
\end{algorithm}

Algorithm~\ref{alg:worklistalg} shows the BBDFGS algorithm~\cite{BBDFGS15}.
%(Recall $X_p$ and $X_k$ denote the set of public and private input variables respectively.)
${\tt check}_{X_p,X_k}$ takes a worklist of pairs $((d_j,E_j)_{0\leq j< n})$ as input
and checks whether every $Z=\bigcup_{0\leq j<n} Z_j$ with $Z_j\in {\mathcal{P}}_{\leq d_j}(E_j)$
is (statistically) independent of $X_k$,
where ${\mathcal{P}}_{\leq d_j}(E_j)$ denotes the set of subsets of $E_j$ with size up to $d_j$,
and ${\tt check}_{X_p,X_k}$ is invoked with the list
$((d, X_o))$ for checking order-$d$ security.

Algorithm~\ref{alg:worklistalg} works as follows. (This represents our interpretation.)
\begin{enumerate}[topsep=1pt,leftmargin=*]
  \item At Line 3, it chooses a subset $Y_j$ with size no larger than $d_j$ from the set $E_j$ for every pair $(d_j,E_j)$
in the worklist.
%
  \item At Lines 4-5, it checks whether the set $\bigcup_{0\leq j< n}Y_j$ is (statistically) independent from $X_k$  by invoking
the procedure ${\tt NI}_{X_p,X_k}$. It raises the error:
${\tt CannotProve}(\bigcup_{0\leq j< n}Y_j)$ if ${\tt NI}_{X_p,X_k}$ fails to prove that;
 Otherwise, $\vec{h}$ is the proof.
%
  \item At Line 6, for each pair $(d_j,E_j)$ in the worklist,
 it tries to add new elements $e\in E_j\setminus Y_j$ to
$Y_j$ by the function ${\tt extend}_{X_p,X_k}$. For each such element $e$,
if it can be proved that $\{e\}\cup\bigcup_{0\leq j< n}Y_j$ is (statistically) independent from $X_k$
using the same proof $\vec{h}$, then $e$ is added to $Y_j$. %, otherwise not.
%Finally,
$\widehat{Y_j}$ denotes the resulting set $Y_j$.
%
  \item At Line 7, ${\tt check}_{X_p,X_k}$ is recursively invoked to check the worklist $(d_j,E_j\setminus \widehat{Y_j})_{0\leq j< n}$.
%
  \item At Lines 8-9, for every  $j$ and $0<i_j< d_j$,
  ${\tt check}_{X_p,X_k}$ is invoked with the updated worklist.
[Note that in the paper \cite{BBDFGS15}, ${\tt check}_{X_p,X_k}(i_j,(\widehat{Y_j}, d_j-i_j,E_j\setminus \widehat{Y_j}))$ is used at Line 9.
It has been changed to ${\tt check}_{X_p,X_k}((i_j,\widehat{Y_j}), (d_j-i_j,E_j\setminus \widehat{Y_j}))$
 in the paper \cite{BBDFGSZ16} (cf.\ Algorithm 11, Line 9) by some same authors. Obviously this is merely a typo in writing.]
\end{enumerate}

Theorem 3  of the paper~\cite{BBDFGS15} claimed the soundness of the BBDFGS Algorithm as follows.
From this Theorem, if ${\tt check}_{X_p,X_k}((d,\{\Expr(x)\mid x\in X_o\}))$ succeeds,
then one can conclude that the program $P$ is order-$d$ secure.

\noindent\fbox{
\begin{minipage}{38em}
Given a program $P$ annotated with the public ($X_p$),
the private ($X_k$), and the random ($X_r$) input variables,
for every integer $d>0$ and a set of expressions $E$,
if ${\tt check}_{X_p,X_k}((d, E))$ succeeds, then every $Z\in {\mathcal{P}}_{\leq t}(E) $ is
(statistically) independent from $X_k$.
\end{minipage}
}

Unfortunately, we have found two issues in this algorithm.

%\subsubsection{Issues}
 \medskip
\noindent{\bf First (minor) issue.} As mentioned on Page 7 of the paper~\cite{BBDFGS15},
  $\mathcal{P}_{\leq t}(X)$ denotes the set of subsets whose size is no larger than $t$.
  Consider the case that $\widehat{Y_j}=\emptyset$ for all $j:1\leq j< n$ (i.e., all the observable variables are not first-order secure).
  Then, an infinite recursion occurs at Line 7. We believe that it is a typo in \cite{BBDFGS15}:
  $\mathcal{P}_{\leq d_j}(E_j)$ should be $\mathcal{P}_{d_j}(E_j)$ in Algorithm~\ref{alg:worklistalg},
  as it is $\mathcal{P}_{d_j}(E_j)$ which is used in the follow-up paper~\cite{BBDFGSZ16}.

 % We finally remark that if the BBDFGS algorithm uses  $\mathcal{P}_{\leq d_j}(E_j)$ instead of
 % $\mathcal{P}_{d_j}(E_j)$,
 However, %the second issue would not occur, i.e., the algorithm would not miss any observable set, although the algorithm might not terminate.
 this is not a salient fix, as it would introduce the second issue, as discussed below.
%   We guess that the second issue may be introduced due to the first minor issue.


\medskip
\noindent{\bf Second (and more serious) issue.}
The worklist checked at Line 9 of Algorithm~\ref{alg:worklistalg}, i.e.,
\begin{center}
${\tt check}_{X_p,X_k}((i_j,\widehat{Y_j}), (d_j-i_j,E_j\setminus \widehat{Y_j}))$
\end{center}
is not sound at least in theoretical. According to what is stated in the paper~\cite{BBDFGS15},\\
\fbox{\begin{minipage}{38em}
Unless otherwise specified, we lift algorithms seen so far to
work with vectors or sets of arguments by applying them element by element.
Note in particular, that the for loop at line 8 iterates over all vectors of $n$ integers
such that each element $i_j$ is \emph{strictly} between $0$ and $d_j$.
\end{minipage}}\medskip

\noindent
We may interpret the worklist $((i_j,\widehat{Y_j}), (d_j-i_j,E_j\setminus \widehat{Y_j}))$ at Line 9, in the following two ways:
\begin{enumerate}
  \item $((i_j,\widehat{Y_j}), (d_j-i_j,E_j\setminus \widehat{Y_j}))_{0\leq j<n}$,
  \item  $((i_j,\widehat{Y_j}), (d_j-i_j,E_j\setminus \widehat{Y_j}), (i_{j'},E_j')_{0\leq j'\neq j<n})$.
\end{enumerate}
However, we believe neither of them is correct, as they may miss some observable sets.


Assume that $\bigcup_{1\leq j<n}\widehat{Y_j}$ is secure, the worklist $(d_j,E_j\setminus \widehat{Y_j})_{0\leq j< n}$ is also correctly checked
at Line 7, and all the recursive calls at Line 9 are finished.
Let us consider the case that
$| E_j \setminus \widehat{ Y_j }|\geq d_j$.
Let $Z=\bigcup_{0\leq j<n} Z_j$ with $Z_j\in \mathcal{P}_{d_j}( E_j )$
such that $Z$ contains $d_j$ elements from $ E_j \setminus \widehat{ Y_j }$, but $Z\cap \widehat{ Y_j }=\emptyset$.
Then, $X\not\subseteq \bigcup_{1\leq j<n}\widehat{ Y_j }$.
Moreover, $Z$ may not be checked in any of the recursive calls at Line 9 (no matter which interpretation is taken),
as $(d_j-i_j, E_j \setminus \widehat{ Y_j })$ is added into the worklist at Line 9, but $i_j>0$ (cf. Line 8)
and {\tt choose} will only choose $d_j-i_j<d_j$ elements from $ E_j \setminus \widehat{ Y_j }$ at Line 3
in the recursive calls.
We could give concrete examples to trigger this issue,
but we believe that the above abstract example suffices to demonstrate.
%Therefore, Algorithm~\ref{alg:worklistalg} indeed is unsound.


Concretely, Algorithm~\ref{alg:worklistalg} is correct for the first-order case under both interpretations.
For the second-order case however, both interpretations are incorrect, which is illustrated in Figure~\ref{fig:Order-2}.

In Figure~\ref{fig:Order-2}, ${\tt check}_{X_p,X_k}((2,E))$ is first invoked.
Assume that $(X_k,X_p) \vdash\widehat{Y}_0^0$ is valid after Line 6
and ${\tt check}_{X_p,X_k}((2,E\setminus\widehat{Y}_0^0))$ succeeds at Line 7.
Then, ${\tt check}_{X_p,X_k}((1,\widehat{Y}_0^0\setminus \widehat{Y}_0^1)(1,(E\setminus\widehat{Y}_0^0)\setminus \widehat{Y}_1^1 ))$
is invoked at Line 9.
In the second recursion, assume that $(X_k,X_p) \vdash \widehat{Y}_0^1 \cup \widehat{Y}_1^1$ is valid after Line 6
and ${\tt check}_{X_p,X_k}((1,\widehat{Y}_0^0\setminus \widehat{Y}_0^1)(1,(E\setminus\widehat{Y}_0^0)\setminus \widehat{Y}_1^1 ))$
succeeds, then the program terminates.
One can observe that neither
$${\tt check}_{X_p,X_k}((1,\widehat{Y}_0^1)(1,(E\setminus\widehat{Y}_0^0)\setminus \widehat{Y}_1^1 ))$$ nor
${\tt check}_{X_p,X_k}((1,\widehat{Y}_0^0\setminus \widehat{Y}_0^1)(1,\widehat{Y}_1^1 ))$ is invoked, which results in the incorrectness of Theorem 3.
Therefore, the BBDFGS algorithm may not be sound  as it stands.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.86\textwidth]{figs//order-2}
  \caption{Illustration for second-order}\label{fig:Order-2}
\end{figure}


%\subsection{Discussion}

%In summary, using $\mathcal{P}_{\leq d_j}(E_j)$ would cause infinite recursion whereas using $\mathcal{P}_{d_j}(E_j)$ would miss observable variables, so
%We mainly focus on the second issue %, as we believe that the first issue should be a typo in \cite{BBDFGS15}.
%Due to the second issue,
%under which
%a ``proved" program may not be secure.
This algorithm was also leveraged
for proving strong non-interference (SNI, \cite{BBDFGSZ16}) of masked programs
and the issue stays. Both algorithms were implemented in the framework provided by \textsf{EasyCrypyt}.
The source code of \cite{BBDFGS15} and \cite{BBDFGSZ16} is not publicly available, which precluded us from
examining how the algorithm is actually implemented.

 % We finally remark that if the BBDFGS algorithm uses  $\mathcal{P}_{\leq d_j}(E_j)$ instead of
% $\mathcal{P}_{d_j}(E_j)$,
%However, the second issue would not occur, i.e.,


%, although the algorithm might not terminate.  We guess that the second issue may be introduced due to the first minor issue.

We note that, these two algorithms were also leveraged very recently in
the \textsf{maskVerif} framework which is publicly available~\cite{BBFG18} with practical optimizations to improve verification time
and extensions of leakage models.
We have examined the code of \textsf{maskVerif}
and did not find the issue. However, as \textsf{maskVerif} is limited to
Boolean programs, so it is not clear at all that, for arithmetic programs, this issue has been fixed, %due to that
%the authors are already aware of this,
or simply is a presentation problem of the papers \cite{BBDFGS15,BBDFGSZ16}.
%or the optimizations of the algorithm.
Nevertheless, this issue has not been reported
formally in literature which may impede reproducing or leveraging their algorithm. (We believe it is a technical issue, and by no means invalidate the general framework \cite{BBDFGS15, BBDFGSZ16} or  their importance and contributions to the formal verification of higher-order masked arithmetic programs.)





%\tl{but this is a different issue?}
%On a different matter, even these issues are correctly fixed, a secure program may still fail to pass the verification, because the  BBDFGS algorithm is incomplete.
%As an example, the program in Figure~\ref{fig:Runningexample} is first-order secure, but not
%second-order secure. This claim cannot be proved using their algorithms, or other existing algorithms. \tl{it is not quite clear}

